Concentrated Differential Privacy for Bandits

Bandits serve as the theoretical foundation of sequential learning and an algorithmic foundation of modern recommender systems. However, recommender systems often rely on user-sensitive data, making privacy a critical concern. This paper contributes to the understanding of Differential Privacy (DP) in bandits with a trusted centralised decision-maker, and especially the implications of ensuring zero Concentrated Differential Privacy (zCDP). First, we formalise and compare different adaptations of DP to bandits, depending on the considered input and the interaction protocol. Then, we propose three private algorithms, namely AdaC-UCB, AdaC-GOPE and AdaC-OFUL, for three bandit settings, namely finite-armed bandits, linear bandits, and linear contextual bandits. The three algorithms share a generic algorithmic blueprint, i.e. the Gaussian mechanism and adaptive episodes, to ensure a good privacy-utility trade-off. We analyse and upper bound the regret of these three algorithms. Our analysis shows that in all of these settings, the prices of imposing zCDP are (asymptotically) negligible in comparison with the regrets incurred oblivious to privacy. Next, we complement our regret upper bounds with the first minimax lower bounds on the regret of bandits with zCDP. To prove the lower bounds, we elaborate a new proof technique based on couplings and optimal transport. We conclude by experimentally validating our theoretical results for the three different settings of bandits.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> proofs/kl_decomposition.tex <==
\section{Lower bounds via couplings for concentrated DP}\label{sec:couplings}
In this section, we are interested in controlling the distance (the Kullback-Leibler, i.e. KL) between marginal distributions induced by a differentially private mechanism, when the datasets are generated using two different distributions. This type of information-theoretic bounds is generally the main step for many standard methods for obtaining minimax lower bounds. Our main theorem in this section relates the effect of Concentrated DP on this information-theoretic quantity. 

In particular, if $\cP_1$ and $\cP_2$ are two data-generating distributions over $\CX^n$, we are interested in the marginals over the output of the mechanism $\mech$ when the inputs are generated from $\cP_1$ and $\cP_2$, i.e. for $\nu \in \{1, 2\}$ and $ A \in \cF$
\begin{equation}\label{eq:marginal_2}
    M_\nu(A) \defn \int_{d \in \CX^n } \mech\left(A \mid d\right) d\cP_\nu\left(d\right)
\end{equation}

In the following, we will provide general results to bound the KL divergence between the distributions $M_1$ and $M_2$ defined in (\ref{eq:marginal_2}), when the mechanism $\mech$ is $\rho$-zCDP. The upper bound depends on the privacy budget $\rho$ and the per-step total variation distance between the data-generating distributions $\cP_1$ and $\cP_2$.

We recall the definition of an $f$-divergence.

\begin{definition}[$f$-divergence]
     Let $f:(0, \infty) \rightarrow \mathbb{R}$ be a convex function with $f(1)=0$. Let $P$ and $Q$ be two probability distributions on a measurable space $(\mathcal{X}, \mathcal{F})$. If $P \ll Q$ then the $f$-divergence is defined as
$$
D_f(P \| Q) \triangleq \mathbb{E}_Q\left[f\left(\frac{d P}{d Q}\right)\right]
$$
where $\frac{d P}{d Q}$ is a Radon-Nikodym derivative and $f(0) \triangleq f(0+)$.
\end{definition}

\subsection{From the KL to a transport problem}
Let $\cP_1$ and $\cP_2$ two distributions over $\CX^n$. Define $\cC$ as a coupling of $(\cP_1, \cP_2)$, i.e. the marginals of $\cC$ are $\cP_1$ and $\cP_2$. We denote by $\Pi(\cP_1, \cP_2)$ the set of all the couplings between  $\cP_1$ and $\cP_2$. Let $M_1$ and $M_2$ be defined as in (\ref{eq:marginal_2}). We recall the definition of an $f$-divergence.

\begin{theorem}\label{thm:kl_to_tr}
    We have that
     \begin{equation}\label{eq:kl_to_tr}
         D_f(M_1 \| M_2) \leq \inf_{\cC \in \Pi(\cP_1, \cP_2)} \expect_{(d,d') \sim \cC} [D_f(\mech_d \| \mech_{d'})].
     \end{equation}
\end{theorem}

\begin{proof}
    Let $\cC$ be a coupling of $\cP_1$ and $\cP_2$. We provide a visual proof of the theorem. 
    
    First, we recall Theorem~\ref{thm:cond_incr}.

    \begin{figure}[h!]
      \includegraphics[width=\linewidth]{figures/take1.png}
      %\caption{A boat.}
      \label{fig:boat1}
    \end{figure}
    
    If $P_X \stackrel{P_{Y \mid X}}{\longrightarrow} P_Y$ and $P_X \stackrel{Q_{Y \mid X}}{\longrightarrow} Q_Y$, then
    $$
    D_f\left(P_Y \| Q_Y\right) \leq \mathbb{E}_{X \sim P_X}\left[D_f\left(P_{Y \mid X} \| Q_{Y \mid X}\right)\right] .
    $$
    
    
    The idea is to use Theorem~\ref{thm:cond_incr}, where the input is a pair of datasets $(d, d')$ sampled from the coupling $\cC$, the first channel applies the private mechanism to the first dataset, the second channel applies the mechanism to the second dataset. In other words,
    \begin{itemize}
        \item $X= (d,d')$ a pair of datasets in $\cX^n$
        \item the input distribution is $P_X = \cC$ the coupling distribution.
        \item the first channel is the mechanism applied to the first dataset $P_{Y \mid X} = \mech(Y \mid d)$.
        \item the second channel is the mechanism applied to the second dataset $Q_{Y \mid X} = \mech(Y \mid d')$.
        \item Y is the output of the mechanism
    \end{itemize}
    Using this notation, we have that
    \begin{itemize}
        \item $P_Y = M_1$ 
        \item $Q_Y = M_2$
        \item $D_f\left(P_{Y \mid X} \| Q_{Y \mid X}\right) = D_f(\mech_d \| \mech_{d'})$.
    \end{itemize}
    Using Theorem~\ref{thm:cond_incr}, we have that 
    $$
    D_f(M_1 \| M_2) \leq  \expect_{(d,d') \sim \cC} [D_f(\mech_d \| \mech_{d'})].
    $$
    which is true for every coupling $\cC$. Taking the infimum over the couplings concludes the proof.

    % Another way to prove this theorem is using the convexity of $f$-divergences.

    
\end{proof}

We will use the group privacy to upper bound the RHS of Equation~\ref{eq:kl_to_tr}.
\begin{theorem}[Group Privacy for $\rho$-zCDP, Proposition 27, \cite{ZeroDP}]\label{thm:grp_priv}
    If $\mech$ is $\rho$-CDP, then
    \begin{equation*}
        \forall d, d' \in \cX^n, ~ \forall \alpha \geq 1, ~ D_{\alpha}(\mech_d \| \mech_{d'}) \leq \rho \dham(d, d')^2 \alpha.
    \end{equation*}
\end{theorem}

Combining the last two theorems gives the following corollary.
\begin{corollary}\label{crl:kl_bound}
    If $\mech$ is $\rho$-CDP, then
    \begin{equation*}
        \KL{M_1}{M_2} \leq \rho \inf_{\cC \in \Pi(\cP_1, \cP_2)} \expect_{(d,d') \sim \cC} [\dham(d, d')^2].
    \end{equation*}
          
\end{corollary}

\begin{proof}
    Let $\mech$ be $\rho$-CDP. 
    Applying Theorem~\ref{thm:kl_to_tr}, with $f(x) = x \log(x)$ gives that
    \begin{equation*}
        \KL{M_1}{M_2} \leq \rho \inf_{\cC \in \Pi(\cP_1, \cP_2)} \expect_{(d,d') \sim \cC} [\KL{\mech_d}{\mech_{d'}}].
    \end{equation*}

    Applying Theorem~\ref{thm:grp_priv} with $\alpha = 1$ gives that
    \begin{equation*}
        \KL{\mech_d}{\mech_{d'}} \leq \rho \dham(d, d')^2
    \end{equation*}

    Combining both inequalities gives the final bound.
\end{proof}

\subsection{Proxy solution to the transport Problem}
Deriving the sharpest upper bound for the KL would require solving the transport problem
\begin{equation*}
    \inf_{\cC \in \Pi(\cP_1, \cP_2)} \expect_{(d,d') \sim \cC} [\dham(d, d')^2].
\end{equation*}

As a proxy, we will use maximal couplings.

\begin{proposition}
    Let $\cP_1$ and $\cP_2$ be two probability distributions that share the same $\sigma$-algebra. There exists a coupling $c_\infty(\cP_1, \cP_2) \in \Pi(\cP_1, \cP_2)$ called a maximal coupling, such that 
    \begin{equation*}
        \expect_{(X_1, X_2) \sim c_\infty(\cP_1, \cP_2)}\left[\ind{X_1 \neq X_2}\right] = \TV{\cP_1}{\cP_2}
    \end{equation*}
\end{proposition}

Using maximal coupling for data-generating distributions that are product distributions yields the following bound.

\begin{reptheorem}{thm:zcdp_deco}[KL decomposition for $\rho$-zCDP]
    Let $\cP_1$ and $\cP_2$ be two product distributions over $\cX^n$, i.e. $\cP_1 = \bigotimes_{i = 1}^n p_{1,i}$ and $\cP_2 = \bigotimes_{i = 1}^n p_{2,i}$, where $p_{\nu,i}$ for $\nu \in \{1, 2\}, i \in [1, n]$ are distributions over $\cX$. Let $t_i \defn \TV{p_{1,i}}{p_{2,i}}$.    
    If $\mech$ is $\rho$-zCDP, then
    \begin{equation*}
        \KL{M_1}{M_2} \leq \rho \left(\sum_{i =1 }^n t_i \right) ^2 + \rho  \sum_{i = 1}^n t_i (1 - t_i)
    \end{equation*}
\end{reptheorem}
   
\begin{proof}
    Let $c_\infty^i$ be a maximal coupling between $p_{1,i}$ and $p_{2,i}$ for all $i \in [1,n]$. We define the coupling $\cC_\infty \defn \bigotimes_{i = 1}^n c_\infty^i$. Then $\cC_\infty$ is a coupling of $\cP_1$ and $\cP_2$.

    Since $\dham(d, d') = \sum_{i=1}^n \ind{d_{i} \neq d'_{i} }$ we get that, for $(d, d') \sim \cC_\infty$,
    $$ \dham(d, d') \sim \sum_{i = 1}^n \text{Bernoulli}( t_i ),$$
    where $t_i \defn \TV{p_{1,i}}{p_{2,i}}$.
    
    This further yields
    
     $$\expect_{(d,d') \sim \cC_\infty} [\dham(d, d')^2 ] =  \left(\sum_{i =1 }^n t_i \right) ^2 + \sum_{i = 1}^n t_i (1 - t_i).$$

    Corollary~\ref{crl:kl_bound} concludes the proof.
\end{proof}

\noindent \textbf{Comments on the bound of Theorem~\ref{thm:zcdp_deco}.} 
This is a centralised $\rho$-zCDP version of the KL-decomposition lemma under local DP~\citep[Theorem 1]{duchi2013local}, and a $\rho$-zCDP version of the Sequential Karwa-Vadhan lemma~\citep{azize2022privacy}. We also refer to~\citep{lalanne2022statistical} that uses similar coupling ideas to derive $\rho$-zCDP variants of LeCam and Fano inequalities.
    


==> proofs/reviews.tex <==
\section{Reviews from the last submission}\label{app:reviews}

\subsection{Meta-review}
While this paper makes valuable contributions to differential privacy in bandits, reviewers raised several common concerns regarding: (i) the problem definition and the use of approximate DP; (ii) the implication of the theorem statements and the roles of $\rho$ and $\horizon$ ; (iii) some steps in the proofs (e.g., the use of the oracle argument). Given these concerns of the reviewers, the paper has to undergo a significant revision before it can be accepted at a future conference.


\subsection{First Review}
This paper presents a comprehensive study on differential privacy for bandits, with a primary focus on zero concentrated differential privacy (zCDP). The authors investigate both worst-case and problem-dependent lower bounds of regret.

Regarding multi-armed bandits, the authors propose an innovative approach called AdaC-UCB, which is shown to be near minimax and problem-dependent optimal. Additionally, for linear bandits, they introduce the AdaC-GOPE algorithm, leveraging G-optimal design and the elimination idea, which also achieves near optimality.

\textbf{Strengths:}
This paper offers a comprehensive investigation of differential privacy for bandits, encompassing both multi-armed bandits and linear bandits. It provides rigorous analysis of lower and upper bounds, supported by experimental evidence. The combination of theoretical results and empirical evaluations enhances the robustness of the findings, making this study valuable for the field of differential privacy in bandit settings.

\textbf{Weaknesses:}
While the paper makes valuable contributions, there are several points that require clarification and improvement:

1: In Definition 1, the authors introduce the bandit adversary protocol, which raises concerns about the potential mismatch between the algorithm's chosen $o_t$ action and the actual feedback given by the adversary's recommended action $a_t$. This discrepancy prompts questions about the regret definition in Equation (2). If the adversary consistently suggests suboptimal arms, the regret would be $\bigO(T)$, implying that $\rho$-zCDP may lead to $\bigO(T)$ regret.

2: It is recommended to use $d_t$ instead of $d$ in Definition 1 to clarify the temporal aspect and avoid potential confusion.

3: The problem-dependent lower bound presented in the paper is meaningless and potentially misleading. As it stands, the asymptotic lower bound indicates a regret of $\Omega(\sqrt{log(T)})$, while the well-known asymptotic regret for bandits is typically $C \log(T)$, where $C$ is a constant.

4: For linear bandits, utilizing G-optimal design with an infinite arm set may result in significant computational overhead. The authors should explore and discuss possible optimizations or approximations to make this approach more practical and efficient.

5: To provide a better evaluation of the proposed methods, the inclusion of baseline algorithms in the experimental section is essential. Comparing the performance of AdaC-UCB and AdaC-GOPE against existing state-of-the-art methods would help readers gauge their effectiveness and gain insights into their advantages and limitations.

6: The motivation example presented in the paper may not be entirely reasonable. To make the paper more relevant and appealing, it is advisable to consider privacy protection for both rewards and actions, as this better aligns with practical applications.

\textbf{Questions:}
See the weaknesses.

\subsection{Second Review}
The paper discusses the concept of multi-armed bandit, which is a type of reinforcement learning consisting of K actions corresponding to K unknown reward distributions. The goal of the policy is to maximize the cumulative reward or minimize the regret. The paper investigates privacy in bandits with a trusted centralized decision-maker through the lens of interactive Differential Privacy (DP). It provides minimax and problem-dependent lower bounds on regret for finite-armed and linear bandits, which quantify the cost of zero Concentrated DP (zCDP) in these settings. The paper proposes two zCDP bandit algorithms, AdaC-UCB and AdaC-GOPE, for finite-armed and linear bandits respectively. Finally, the paper provides experimental validation of the theoretical results under different settings.


\textbf{Strengths:}
Clean exposition of the problem formulation, motivation, results, and algorithm.
Handling bandits problem under zCDP.
Provide regret minimax and problem-dependent lower bounds on regret for both MAB and linear bandits.

\textbf{Weaknesses:}
I have some concerns about if it is necessary to study the problem under approximation DP since bandits and linear bandits have been studied under pure DP.
The novelty of algorithms are highly similar to the algorithm in [1]. 

\textbf{Questions:}
Why do you consider approximation DP? Since the Gaussian mechanism is better than the Laplacian mechanism under high dimension case. But for the finite-armed case, is it necessary?
Could you please clarify the novelty of the algorithms compared with algorithms in [1].
Doubling and forgetting techniques have been used in previous bandits. And high-privacy regimes and low-privacy regimes have been proposed in [1]. What is the main difference between the work and [1].

[1]. Azize, A. and Basu, D. (2022). When privacy meets partial information: A refined analysis of differentially private bandits. arXiv preprint arXiv:2209.02570.

\subsection{Third review}
This paper investigates privacy concerns in bandit algorithms used in interactive learning and recommender systems, where sensitive user data is often involved. Focusing on bandits with a trusted centralized decision-maker, the study explores privacy through interactive Differential Privacy (DP), specifically zero Concentrated DP (zCDP). The paper establishes lower bounds on regret for finite-armed and linear bandits, shedding light on the trade-off between privacy and performance. Additionally, two $\rho$-global zCDP bandit algorithms, AdaC-UCB and AdaC-GOPE, are proposed and analyzed. Experimental validation supports the theoretical findings, showcasing the effectiveness of the algorithms in maintaining privacy while minimizing regret.

\textbf{Strengths:}
Establish the lower bounds for zero-concentrated DP, which seems to be the first result under this notion.
Provide algorithms that are able to achieve minimax regret bound

\textbf{Weaknesses:}
The introduction of interactive DP is not well justified, in particular, the comparison with adaptivity in DP is missing
Some of the details in the proofs are not clear (see my questions below)
The proposed algorithms are quite standard, which follow more or less the same idea as previous works

\textbf{Questions:}
It seems to me that the main motivation of interactive DP is to handle the possible adversarially selected feedback (i.e., instead of returning the reward of an action selected by the policy, it can return the reward of another action). If this understanding is correct, I did not see the key difference compared to the standard DP + adaptivity. That is, by standard DP, the adversary could also be all other users and they can collude together (by specifying their reward tape) to infer one particular user. Also, for standard DP bandits, it is not one shot as claimed by the authors. Rather, all other users can be adaptive. In sum, it is unclear to me that the importance/necessity of introducing interactive DP for bandits. As a side note, the original papers on interactive DP mainly aim to handle the concurrent composition of interactive mechanisms. They also mention that the traditional adaptive mechanism is one particular interactive mechanism. Their main contribution is to handle the composition of multiple interactive mechanisms.

Can you authors explain line 512-513, i.e., 
$\mathcal{V}^\pi_r (a^\horizon)$. Why does this hold? In particular, if I understand it correctly, 
$\mathcal{V}^\pi_r (a^\horizon)$ is the probability of producing  $a^\horizon$ given the reward sequence $(r_1, \dots r_\horizon)$ . The authors seem to use some conditional independence here. But, if one condition on future reward, the probability of current action selection is different? To some extent, this view-DP may not make sense. Note that when I checked the references, I found that (Mishra and Thakurta, 2015) in fact adopt table rewards for DP definition (rather than view DP based on rewards) and (Tossou and Dimitrakakis, 2016) define its DP without condition on all reward sequences, i.e., for each $t$, it condition only on history $t-1$.

Similar questions as the above apply to line 547, line 661/662.

I have some concerns about Step 3 in the proof of Theorem 2. First, the Oracle argument in Shariff and Sheffet, 2018 applies to a fixed number of samples, which is fine. However, in Step 3, the proof requires the Oracle to provide $n_a$  in expectation, which is unclear to me. That is, whether this will cause any subtle issues, noting Theorem 1 holds only for a constant number of samples $n$, i.e., no additional randomness depends on samples.

What's the purpose of Lemma 6? If I understand it correctly, it is mainly used to handle the correlation in sequential decision-making. If this is the motivation, then does this mean that the proof in Azize and Basu, 2022 (for linear bandit under pure DP) is not correct? That is, in Azize and Basu, 2022, the proof directly uses the KL divergence for product distributions, which is not the case anymore in the linear bandit setting.

Why not directly use Lemma 6 to prove Theorem 2, which helps to avoid the Oracle argument and handles the correlation naturally?

Question about Lemma 1: I roughly know the proof idea behind it. But, I still have some concerns. That is, can one copy the reward K times? Suppose I have two arms, i.e., arm 1 with a mean 0 and arm 2 with a mean 1 (both are Ber distributions). Then, one cannot copy the reward 0 to arm 2?

Question about Lemma 3: On a high level, I know the difference between pure DP and approximate DP, i.e., whether one can only focus on a single outcome or not. However, I have some concerns about Lemma 3. Let us consider $T=2$ and the following specific policy $\pi$: on round $t = 1$, it uniformly selects an arm from $\arms$ arms; on round $t = 2$, its output satisfies $(\epsilon, \delta)$-DP $\delta >0$ with respect to the reward on round $t = 1 $. Then, for any event $E$ at round $t = 2$ and for any neighboring table rewards $d$, $d'$ , the output of this policy is still $(\epsilon, \delta)$-DP (rather than  $K \delta$). This holds since the output distribution at $t = 2$ is "close" for any event $E$ and any neighboring reward on $t = 1$. One can also extend it to the event $E$ over both rounds, as the first round is trivial DP. This also holds for all $(\epsilon, \delta)$-DP MAB algorithm. My main point is that it seems that as long as one algorithm is $(\epsilon, \delta)$-DP with respect to any neighboring observed reward sequences, it is also $(\epsilon, \delta)$-DP with respect to table rewards. Do I miss something here? If I understand it correctly, since the information used in policy decisions for MAB is only rewards, it might be the case that view-DP and table-DP are equivalent, even in approximate DP, RDP, zCDP? For instance, if one compares the probability in line 513 and line 547, there seems to be a one-to-one correspondence under neighboring observed rewards and neighboring table rewards?

\subsection{Fourth review}
This paper explores privacy concerns in bandit-based interactive learning and recommender systems with a trusted centralized decision-maker. It focuses on zero Concentrated Differential Privacy (zCDP) and provides minimax and problem-dependent lower bounds on regret for finite-armed and linear bandits. The paper proposes two zCDP bandit algorithms, AdaC-UCB and AdaC-GOPE, and analyzes their regret.


\textbf{Strengths:}
The paper provides minimax and problem-dependent lower bounds on regret for finite-armed and linear bandits

The paper proposes two zCDP bandit algorithms, AdaC-UCB and AdaC-GOPE, specifically designed for finite-armed and linear bandits, respectively. Further, regret is analyzed.

\textbf{Weaknesses:}
Can the result be generalized beyond finite and linear case. For example, if there exist a base algorithm with certain properties, then I can have a DP algorithm?

There has been work using homomorphic encryption on bandits [https://arxiv.org/abs/2103.09927]. Can the authors compare between the approaches and the results.

The challenge due to interaction is unclear. Why does having interaction affect the problem, in the sense that the algorithms could be the same and for achievability, we could have the previous known algorithms?

\textbf{Questions:}
Please see above.

\subsection{Addressing the Reviews in the Current Version}

As suggested by the meta-review, the paper had a major revision compared to the last submission.


1. We study relaxations of DP in bandits as an answer to the open problems in~\cite{dpseOrSheffet, azize2022privacy}. These relaxations are well-studied in the DP literature and provide good privacy guarantees with better utility than pure DP. Our results confirm this general insight for bandits. We explicate this motivation in the Introduction and validate the insights with our results throughout the paper (e.g. Theorem~\ref{thm:grp_priv}, Remark 5, Remark 6 etc.).

2. The new version of the submission compares in depth different types of adaptation of DP to bandits (Sec.\ref{sec:priv_def}), rather than proposing directly the most effective one. We explain the relations between the definitions and the intuition behind defining them with more granularity and in detail. With our rewriting of Section~\ref{sec:priv_def}, we address the confusion due to notation and the multiple interaction processes in Remark 2 (i.e. we explicitly differentiate between two interaction protocols, one for privacy and one for regret). We also add an explicit counter-example explaining why View and Table DP are not exactly equivalent (Prop.~\ref{prop:tab_view}) and also relate Interactive to Table DP (Prop~\ref{prop:int_table}).

3. In algorithm design, we propose and analyse a new algorithm, i.e. \adaroful{} (Algorithm~\ref{alg:rare_lin_ucb}), for linear contextual bandits with context-dependent and (possibly infinite) countable actions.

4. For regret lower bounds, the result on the problem-dependent lower bound for finite-armed bandits has been removed from the paper, since the ``oracle argument" proof lacked rigour. Also, the proof of the minimax lower bound for finite-armed lower bound has been rewritten, again removing the ``oracle argument" proof, and directly using the KL decomposition of Theorem~\ref{lm:kl_decompo_var}. The role of $\rho$ and $T$ in the lower bounds has been explicitly addressed in Remark 6.
